Model Checking Finite-Horizon Markov Chains with Probabilistic Inference

We revisit the symbolic verification of Markov chains with respect to finite horizon reachability properties. The prevalent approach iteratively computes step-bounded state reachability probabilities. By contrast, recent advances in probabilistic inference suggest symbolically representing all horizon-length paths through the Markov chain. We ask whether this perspective advances the state-of-the-art in probabilistic model checking. First, we formally describe both approaches in order to highlight their key differences. Then, using these insights we develop Rubicon, a tool that transpiles Prism models to the probabilistic inference tool Dice. Finally, we demonstrate better scalability compared to probabilistic model checkers on selected benchmarks. All together, our results suggest that probabilistic inference is a valuable addition to the probabilistic model checking portfolio -- with Rubicon as a first step towards integrating both perspectives.

==> dice.tex <==
% The current implementation of dice uses floating point arithmetic. However, the dynamic programming solution of \eqref{eq:bellman} is easily extensible to rationals (or something along those lines)



%\subsection{\dice{}: Constructing Path-Sets Efficiently}

% \begin{figure}
%   \centering
% \begin{lstlisting}
% fun step(state: (bool, bool)) {
%     let s0 = fst state in
%     let s1 = fst (snd state) in
%     if s0 && s1 then 
%        (s0, s2)
%     else
%     let s0p = if s0 then flip 0.1 else flip 0.2 in
%     let s1p = if s1 then flip 0.2 else flip 0.3 in
%     (s0p, s1p)
% }
% let s0 = (false, false) in
% let s0 = step(s0) in
% let s0 = step(s0) in
% (fst s0) && (snd s0)
% \end{lstlisting}
%   \caption{A \dice{} program encoding two parallel chains with finite horizon $h=2$.}
% \end{figure}

% Historically the computation tree has not been explicitly constructed during
% probabilistic model checking. One possible reason is that, from the perspective
% of traditional model checking, the computation tree contains extraneous
% information: retaining the \emph{history} of all possible transitions is not
% relevant in this setting, since the query of interest typically quantifies over
% all possible histories. However, in the probabilistic setting, this history is essential for
% computing the probability distribution over the reachable states.

% In contrast to the model checking community\sj{It is not used in model checkers, that does not mean it is not a common view}, the computation-tree perspective is
% ubiquitous in the artificial intelligence community, which tackles similar
% probabilistic reasoning tasks in the context of Bayesian probabilistic
% inference. 


% - when is BDD small (only touch briefly, keep it concrete)

% - what is dice doing (yes! more of this.)

% - what is new for model checking

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:

